Introduction to localization in quantum field theory

This is the introductory chapter to the volume. We review the main idea of the localization technique and its brief history both in geometry and in QFT. We discuss localization in diverse dimensions and give an overview of the major applications of the localization calculations for supersymmetric theories. We explain the focus of the present volume.

==> PZdef.tex <==
\usepackage{ytableau}
\usepackage[margin=1in]{geometry}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsxtra}
\usepackage{amscd}
\usepackage{xcolor}
\usepackage{tikz-cd}
\usetikzlibrary{matrix,arrows,decorations.pathmorphing}
\usepackage[mathscr]{euscript}
\usepackage{amscd}
\usepackage{slashed}
\usepackage{listings}
\usepackage[inline]{showlabels}
\usepackage{graphicx}
\usepackage{todonotes}
\usepackage[pagebackref=false]{hyperref}
\definecolor{darkblue}{RGB}{0,0,192}
\definecolor{darkgreen}{RGB}{0,192,0}
\hypersetup{colorlinks = true,extension = notused,linkcolor = darkblue,anchorcolor = red,citecolor = darkgreen,filecolor = red,pagecolor = red,urlcolor = darkblue}
% \usepackage[numbers,sort&compress]{natbib}
% \usepackage{hypernat}
\usepackage{iftex}
\ifxetex
        \usepackage{fontspec}
        \setmainfont[Ligatures=TeX,Extension=.otf,BoldFont=cmunbx,ItalicFont=cmunti,BoldItalicFont=cmunbi]{cmunrm}
\else
\fi








%%% THEOREMS
% \newtheorem{problem}{Problem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{question}{Question}
 \newtheorem{example}{Example}
% \newtheorem{remark}{Remark}
% \newtheorem{note}{Note}
% \newtheorem{exercise}{Exercise}
        
%%% BRACKETS
\newcommand {\la} {\left \langle}
\newcommand {\ra} {\right \rangle}
\newcommand {\lb} {\left (}
\newcommand {\rb} {\right )}
\newcommand {\lfb} {\left \{}
\newcommand {\rfb} {\right \}}
\newcommand {\lsb} {\left [}
\newcommand {\rsb} {\right]}
\newcommand{\br}[1]{\left( #1 \right)}
\newcommand{\vev}[1]{\left\langle #1 \right\rangle}
\newcommand{\ket}[1]{\left |  #1 \right \rangle}
\newcommand{\bra}[1]{\left \langle  #1 \right |}
\newcommand{\vect}[1]{\overrightarrow{ #1 }}

%%% CAL LETTERS
\newcommand {\CalA} {\mathcal A}
\newcommand {\CalD} {\mathcal D}
\newcommand {\CalE} {\mathcal E}
\newcommand {\CalF} {\mathcal F}
\newcommand {\CalG} {\mathcal G}
\newcommand {\CalH} {\mathcal H}
\newcommand {\CalI} {\mathcal I}
\newcommand {\CalJ} {\mathcal J}
\newcommand {\CalO} {\mathcal O}
\newcommand {\CalZ} {\mathcal Z}
\newcommand {\CalN} {\mathcal N}
\newcommand {\CalC} {\mathcal C}
\newcommand {\CalL} {\mathcal L}
\newcommand {\CalK} {\mathcal K}
\newcommand {\CalM} {\mathcal M}
\newcommand {\CalP} {\mathcal P}
\newcommand {\CalR} {\mathcal R}
\newcommand {\CalS} {\mathcal S}
\newcommand {\CalT} {\mathcal T}
\newcommand {\CalU} {\mathcal U}
\newcommand {\CalV} {\mathcal V}
\newcommand {\CalX} {\mathcal X}
\newcommand {\CalW} {\mathcal W}

%%% BOLD LETTERS
\newcommand {\BB}   {\mathbb B}
\newcommand {\BD}   {\mathbb D}
\newcommand {\BS}  {\mathbb S}
\newcommand {\BI}   {\mathbb I}
\newcommand {\BT}   {\mathbb T}
\newcommand {\BR}   {\mathbb R}
\newcommand {\BZ}   {\mathbb Z}
\newcommand {\BC}   {\mathbb C}
\newcommand {\BN}   {\mathbb N}
\newcommand {\BO}   {\mathbb O}
\newcommand {\BP}   {\mathbb P}
\newcommand {\BQ}   {\mathbb Q}
\newcommand {\BW}   {\mathbb W}
\newcommand {\RP}   {\mathbb R \mathbb P}
\newcommand {\CP}   {\mathbb C \mathbb P}
\newcommand {\Unity}{\mathbf 1}

%%% GREEK LETTERS
\newcommand {\al} {\alpha}
\newcommand {\ald}{\dot \alpha}
\newcommand {\be} {\beta}
\newcommand {\bed} {\dot \beta}
\newcommand {\de} {\delta}
\newcommand {\ve}  {\varepsilon}
\newcommand {\ep}  {\epsilon}
\newcommand {\ka} {\kappa}
\newcommand {\lam}  {\lambda}
\newcommand {\si}   {\sigma}
\newcommand {\sib}  {\bar \sigma}
\newcommand {\thb}  {\bar \theta}
\newcommand {\vphi} {\varphi}
\newcommand {\ze} {\zeta}
\newcommand {\ro} {\rho}
\newcommand {\om} {\omega}

%%% FRAK LETTERS
\newcommand{\g}{\mathfrak{g}}
\newcommand{\h}{\mathfrak{h}}
\newcommand{\frakH}{\mathfrak{H}}
\newcommand{\frakd}{\mathfrak{d}}
\newcommand{\frakk}{\mathfrak{k}}
\newcommand{\frakl}{\mathfrak{l}}

%%% DERIVATIVES
\newcommand{\Dslash}{\ensuremath \raisebox{0.025cm}{\slash}\hspace{-0.25cm} D}


%%% OPERATORS
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\td}{td}
\DeclareMathOperator{\eu}{eu}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\spanlin}{span}
\DeclareMathOperator{\Map}{Map}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\coKer}{coKer}
\DeclareMathOperator{\Img}{Img}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\tr} {tr}
\DeclareMathOperator{\Tr} {Tr}
\DeclareMathOperator{\str} {str}
\DeclareMathOperator{\rk} {rk}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\HH} {HH}
\DeclareMathOperator{\Pexp} {Pexp}
\DeclareMathOperator{\ad} {ad}
\DeclareMathOperator{\ind} {ind}
\DeclareMathOperator{\Id} {Id}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\codim}{codim}



\newcommand{\SU}{SU}
\newcommand{\SO}{SO}
\newcommand{\Spin}{Spin}
\newcommand{\Sp}{Sp}
\newcommand{\OSp}{OSp}
\newcommand{\GL}{GL}
\newcommand{\SL}{SL}
\newcommand{\PSL}{PSL}
\newcommand{\PSU}{PSU}
\newcommand{\Cl}{\mathrm Cl}
\newcommand{\spin}{\mathfrak {spin}}
\newcommand{\sog}{\mathfrak {so}}
\newcommand{\osp}{\mathfrak {osp}}
\newcommand{\spn}{\mathfrak {sp}}
\newcommand{\su}{\mathfrak {su}}
\newcommand{\un}{\mathfrak {u}}
\newcommand{\sln}{\mathfrak {sl}}

%%%OTHER
\newcommand{\const}{\mathrm{const}}


\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{http://arxiv.org/abs/#1}}
\newcommand{\libs}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/spires/#1}{\nolinkurl{#1}}}
\newcommand{\libm}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/math/#1}{\nolinkurl{#1}}}
\newcommand{\libt}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/talks/#1}{\nolinkurl{#1}}}
\newcommand{\libb}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/books/#1}{\nolinkurl{#1}}}
\newcommand{\libr}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/research/#1}{\nolinkurl{#1}}}
\newcommand{\libn}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/research/_notes/#1}{\nolinkurl{#1}}}
\newcommand{\libp}[1]{\href{file://localhost/Users/pestun/Dropbox/lib/pestun/#1}{\nolinkurl{#1}}}
\newcommand{\myref}[1]{[notes #1]}








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 
\numberwithin{equation}{section}

